Seamless Human Motion Composition with Blended Positional Encodings

Conditional human motion generation is an important topic with many applications in virtual reality, gaming, and robotics. While prior works have focused on generating motion guided by text, music, or scenes, these typically result in isolated motions confined to short durations. Instead, we address the generation of long, continuous sequences guided by a series of varying textual descriptions. In this context, we introduce FlowMDM, the first diffusion-based model that generates seamless Human Motion Compositions (HMC) without any postprocessing or redundant denoising steps. For this, we introduce the Blended Positional Encodings, a technique that leverages both absolute and relative positional encodings in the denoising chain. More specifically, global motion coherence is recovered at the absolute stage, whereas smooth and realistic transitions are built at the relative stage. As a result, we achieve state-of-the-art results in terms of accuracy, realism, and smoothness on the Babel and HumanML3D datasets. FlowMDM excels when trained with only a single description per motion sequence thanks to its Pose-Centric Cross-ATtention, which makes it robust against varying text descriptions at inference time. Finally, to address the limitations of existing HMC metrics, we propose two new metrics: the Peak Jerk and the Area Under the Jerk, to detect abrupt transitions.

==> sections/6_extra_material.tex <==


%=========================================

\section{Supplementary material}

%=========================================


\subsection{Related work on positional encodings}
\label{subsec:supp_related_pe}
blah blah

%=========================================

\subsection{Details on datasets and evaluation}

Additionally, we sample text combinations to represent different composition scenarios and needs. For HumanML3D, we build 4 subsets with mixed random (3-10s), short (3-5s), medium (5-8s), and long (8-10s) test subsequences. For Babel, half of the evaluation sequences are sampled from the consecutive textual descriptions present in the test set, and the remaining sequences are randomly sampled so that consecutive textual descriptions do not appear together neither in the training nor in the test set.

%=========================================

\subsection{Models and training details}
\label{subsec:supp_training_details}

Tricks and other cool stuff

\begin{itemize}
    \item We need to disallow attention with keys inside the padding that homogenizes sequences in MDM. It breaks locality and translation invariance (it memorizes end-of-sequence position even locally).
    %\item (NOT WORKING VERY WELL) We also need to apply random attention span trimming. We can't allow the model to infer where the sequence ends easily, because in \modelname{}, the action should end once it is done, and not once the end of the sequence is reached.
    \item We need to cap attention to the maximum sequences length seen in training. Otherwise, relative PE reaches out-of-distribution values and generation collapses.
    \item We need to tune the appropriate classifier-free guidance weight. If too high, the action performed inside each subsequence will represent better the text, but have sharper transition with acceleration.
    \item For Babel, training includes combinations of subsequences in order to include more variability of motion. 
\end{itemize}

Regarding the baseline implementations:
\begin{itemize}
    \item \textbf{DoubleTake.} We re-evaluate it with a more fair scenario: \textit{the handshake is added to the samples to be generated}, and not substracted as in the original evaluation. We argue that the original implementation deals with a length gap between ground truth and generated samples.
    \item Diffusion models --> For these, the overlapping transition lengths are set to 20 and 10 frames for HumanML3D and Babel, respectively. Blending values for DoubleTake are set to 10 and 5, respectively.
\end{itemize}

%=========================================

%=========================================

\subsection{Attention scores}
\label{subsec:supp_attention_scores}

It would be interesting to plot the scores in absolute vs. relative attention to check locality assumptions.

%=========================================

\subsection{Condition importance}
\label{subsec:supp_condition_importance}

It would be interesting to show the strength of the motion prior in later denoising stages. There is a tradeoff between condition and motion prior guidances. We can check the effect of dropping the condition in later denoising stages, and the difference between scores (y-axis: $\mid f(x_t, c)-f(x_t, \emptyset)\mid$, x-axis: $t$). Mention that future work could explore schedules for the guidance score along the denoising chain.

Also related, show the attention scores of the condition across the CAT stages.

%=========================================
\subsection{Attention horizon ablation}
\label{subsec:supp_horizon}


\begin{table}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/atthorizon_humanml_results.tex}}
    \caption{humanml atthorizon}
    \label{tab:humanml_atthorizon}
\end{table}

\begin{table}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/atthorizon_babel_results.tex}}
    \caption{babel atthorizon}
    \label{tab:babel_atthorizon}
\end{table}



%=========================================

\begin{table*}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/babel_scenarios.tex}}
    \caption{babel scenarios (in vs. out)}
    \label{tab:babel_scenarios}
\end{table*}


\begin{table*}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/humanml_scenarios.tex}}
    \caption{humanml scenarios (short vs. medium vs. long) \textcolor{red}{Does it make sense to include FID comparison here? meh}}
    \label{tab:humanml_scenarios}
\end{table*}


%=========================================

\subsection{Fine-grained experimental results}
\label{subsec:supp_finegrained_exps}


%=========================================

\subsection{Extrapolation capabilities}
\label{subsec:supp_extrapolation}

Extrapolation \textit{quantitative} results, and mayb also individualized jerk plots?

%=========================================

\subsection{More qualitative results}
\label{subsec:supp_qualitative}

%=========================================

\subsection{Inference time analysis}
\label{subsec:supp_time_analysis}
Not sure about this without a custom kernel implementation... It might be slower :'(

%=========================================



==> sections/7_other_stuff.tex <==

\clearpage

\section{Other stuff}

\subsection{OLD explanation on the role of heterogeneous conditioning}
\def\seq{x}
\def\embseq{E_{\seq}}
\def\cond{c}
\def\embseqc{E_{\seq,\cond}}
(TODO we need to revisit both self-attention-MDM and cross-attention-MotionDiffuse) Let's revisit the standard attention mechanism. We refer to the sequence of pose embeddings of $\seq$ as $\embseq$. Absolute positional encodings are already embedded in $\embseq$ for notation simplicity. When the conditions for each frame $\cond_t$ have been embedded to $\embseq$, we replace it by $\embseqc$. Now, the attention score in the original Transformer~\cite{} is computed as:
\begin{equation}
    (W_q \embseqc)^T(W_k \embseqc)=\embseqc^T W_q^T W_k \embseqc.
\end{equation}

We argue that such definition becomes a limitation for our goal, in which we assume that in training $c_{t_1}= c_{t_2} \; \forall t_1, t_2 \in [0,S)$, i.e., the whole sequence is conditioned on a single condition. In the attention mechanism, the query pose embedding at $t_1$ is multiplied by the key pose embedding at $t_2$. As a result, if $c_{t_1}\neq c_{t_2}$ in training time, the query and key in $t_1$ and $t_2$, respectively, will have never been seen in training, and the resulting attention score will be unreliable, even when $t_1$ and $t_2$ are consecutive poses. This is problematic in our scenario because attending to each token's local neighborhood of poses is important to ensure a smooth and realistic transition. Instead, we propose to embed the condition only to the query. As a result, the attention scores are computed as
\begin{equation}
    \embseqc^T W_q^T W_k \embseq.
\end{equation}

\textcolor{red}{[Do we need to assume from now that $\embseq$ is supervised to correspond to an embedded pose, or is the residual enough???]} %Now, the local neighborhood of any pose token will have similar noisy poses, and therefore similar $\embseq$, thus similar keys. 
With this formulation, let's consider a transition at time $\tau$ where condition $c_{\tau^-}\neq c_{\tau^+}$. When computing the attention scores for a pose token at $t \rightarrow \tau, t<\tau$, $\embseq^{t'}$, it attends to all poses. When attending to $t' \rightarrow \tau^-$, $\embseq^{t'}$ was seen in training. When $t' \rightarrow \tau^+$, $\embseq^{t'}$ still belongs to the noisy poses manifold, and \textcolor{blue}{up to some extent}, it has been seen in training time. Whether or not is important to be attended to will depend on the denoising stage. At initial stages, the noisy poses manifold is close to the Gaussian noise space, and there is almost no out-of-distribution attention pairs. At later stages, when high frequencies recovered, attention is rather local and the continuity and realism of movements is prioritized. Therefore, poses are attended locally and out-of-distribution attention pairs are not problematic.

To solve the issues here explained, we propose to tackle the motion generation problem as a translation problem where each noisy frame is denoised as a responde to the question: given the control signal represented in this frame, and its noisy neighbor poses, which has to be my denoised pose? We argue this is a very convenient framework for naturally modeling transitions. The motion prior is inforced, as neighboring poses are the most powerful source of information at later denoising stages.



\textbf{IDEA:} in transitions, mixing motion from two different movements is not critical because 1) when the noise level is high, the network is very robust to random motion perturbations, and therefore, also to these shifts, and 2) when the noise level is low, the network is only aiming at adding high-resolution details, i.e., local attention (\textcolor{red}{Ideally, we should see how far the network attends depending on the noise level. This would be an extremely valuable analysis.}). 

\subsection{Important questions to be answered (Can be in Supp.)}

\begin{itemize}
    \item \textbf{Q. Why not using an iterative approach with a bit of overlap between segments?} 1) Because those approaches assume the dependencies are only in the transition. This is NOT true in many cases. If the person needs to grab an object, the whole previous 2s might need to approach the object. 2) Because these approaches duplicate the denoising in the overlapped regions, and merge both scores somehow. We don't want that. 3) Because they need to arbitrarily choose a transition length.

    \item \textbf{Q. Why transition is realistic if such transition is not present in any dataset?} Basic motion dynamics are implicitly learnt by any model with sufficient variety in the training data. The iterative nature of diffusion models allows the inference to find the appropriate way to trainsition from one action to another one. 

    \item \textbf{Q. What is the difference w.r.t. inpainting?} With inpainting, one side of the synthesized motion is fixed. If the diffusion model doesn't encode an appropriate transition into such fixed motion, the result will look unnatural. Same thing happens with double-take or other transition-based generation models. In our framework, both processes can benefit from using info from the other one to refine itself later. Anything useful that has been learnt by the model will be retrieved and used in its favor. 

    \item \textbf{Q. What about heteregeneous noise schedules/markov chains across samplers from different models?} This is not a problem. The $x0$ parameterization does the trick. You can use it to move it back to ANY noise level. So both samplers can work at different step-rate and noise schedule.
\end{itemize}



\subsection{\textit{Anything}-to-motion \textcolor{red}{(DON'T KNOW IF ENOUGH TIME)}}

\modelname{}'s combination of generated motions is agnostic to particularities of the models, so it can be used to combine different models. To prove the flexibility of the proposed approach, we combine the following models:

\textbf{Text-to-motion.} MDM~\cite{tevet2022mdm} uses a normalized motion representations where all actors are reshaped to a standard body shape. However, when humans interact with objects, or other humans, they need to be self-aware of their body shape. Otherwise, they can become clumsy. Therefore, we retrain MDM with the non-normalized data.

\textbf{Grab-pose generation.} Options: GOAL (grab generation, GG + deterministic infiller)~\cite{taheri2022goal}, or SAGA (GG + stochastic infiller)~\cite{wu2022saga}. OR just train an MDM for this.

\textbf{Interaction generation.} Options: InterDiff???

\textcolor{red}{BONUS}: if joints are also disentangled (if not too???), then we can even carry objects on while doing other stuff like walking, or jumping.

Constraints:
\begin{itemize}
    \item (YES) Anything as long as it can be transformed to each model's output. Ideal format: SMPL-H/X thetas (axis-angle rep. of body pose and hands angles).
    \item (MAYBE) Model: TO BE EXPLORED, but probably specific to attention-based encoder-only models.
    \item (NO) Condition: can be anything.
    \item (NO) Denoising: anything can be performed between denoising steps.
    \item (NO) Parameterization: in theory, different parameterizations can be used in paralel.
\end{itemize}




\subsection{Mixture of Diffusions}
Define what a Mixture of Diffusions is, and why it works.

The structure of \modelname{} based on cross-frame attention builds a particular diffusion process where the denoising of each frame at time $t$ depends on the denoising state of all other joints/frames at time $t-1$. The length of the temporal dependencies is limited by the length of the longest sequences during training each submodel. As a result, there is no need to overlap denoising processes, and this observation might be the reason why PriorMDM needs to overengineer the transition generation. 

\textbf{Different models.} Our architecture conditions the denoising at every pose on the previous noisy motion. This makes it theoretically suitable for the parallel denoising with several models with different control signals. The only condition would be using the same representations as input.



\begin{table*}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/cfg_babel_results.tex}}
    \caption{babel cfg}
    \label{tab:babel_cfg}
\end{table*}

\begin{table*}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/cfg_humanml_results.tex}}
    \caption{humanml cfg}
    \label{tab:humanml_cfg}
\end{table*}



\begin{table*}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/steps_babel_results.tex}}
    \caption{babel steps}
    \label{tab:babel_steps}
\end{table*}

\begin{table*}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/steps_humanml_results.tex}}
    \caption{humanml steps}
    \label{tab:humanml_steps}
\end{table*}




\begin{table*}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/epochs_humanml_results.tex}}
    \caption{humanml epochs}
    \label{tab:humanml_epochs}
\end{table*}




\begin{table*}[]
    %\small
    \resizebox{\linewidth}{!}{\input{tables/auto/epochs_babel_results}}
    \caption{babel epochs}
    \label{tab:babel_epochs}
\end{table*}





\subsection{Pairing functions}
\label{subsec:supp_pairingf}

To achieve this, we propose to use Rosenberg-Strong pairing function~\cite{}. Such function is a bijective projection $\mathbf{p}:\mathbb{N}\times\mathbb{N}\rightarrow\mathbb{N}$ defined as:
\begin{equation}
    \mathbf{p}(m,n) = (\max(m,n))^2+max(m,n)+m-n.
\label{eq:pairing}
\end{equation}

%The inverse of the Rosenberg-Strong pairing function $r(x,y)$ is:
%\begin{equation}
%    r_2^{-1}(z)=
%    \begin{cases}
%      (z-k^2, k) & \text{if}\;\; z-k^2<k\\
%      (k, k^2+2k-z) & \text{otherwise}
%    \end{cases},      
%\end{equation}
%where $k=\lfloor\sqrt{z}\rfloor$.

However, \autoref{eq:pairing} can not acquire the form of $\mathbf{p}(m,n)=h_q(m)-h_k(n)$ due to the presence of the $\max$ function. Given that $m$ and $n$ are the queries and keys positions, respectively, we can reparameterize $m$ so that $\hat{m}=m+S$, where $S$ is the maximum sequence length expected. Thus, $\hat{m}>n\Rightarrow \max(\hat{m},n)=\hat{m}, \;\forall m,n\in [0, S)$ representing any pair of query/key positions, and \autoref{eq:pairing} becomes:
\begin{equation}
    \mathbf{p}(m,n) = 
    \hat{m}^2+2\hat{m}-n =
    \underbrace{(m+S)^2+2(m+S)}_{h_q(m)}
    -
    \underbrace{n}_{h_k(n)}
\label{eq:pairing_reparam}
\end{equation}

Now, we can define the absolute rotary PE as a reparameterization of the relative rotary PE defined in \autoref{eq:relative_rope}:
\begin{equation}
    \langle f_q(x_m, h_q(m)), f_k(x_n, h_k(n))\rangle = g(x_m, x_n, \mathbf{p}(m, n))
\end{equation}



\subsection{Sampling at inference}
\label{subsec:supp_sampling}

\begin{itemize}
    %\item \textbf{Sequential.} At each denoising step $t$, each motion segment is denoised individually conditioned on that specific $c_i$. For next denoising step $t+1$, denoised poses from all models are concatenated, $\hat{x}_0^t$ and diffused into $x_{t+1}$. This is equivalent to performing inpainting at each denoising step.
    \item \textbf{Parallel - $O(n)$.} At each denoising step $t$, each motion segment is conditioned on its respective $c_i$. Of course, this is not suitable when using $K\geq 1$ models, or when using a single model without \textit{token-wise conditioning} (e.g., MDM).
    \item \textbf{Mixed - $O(Kn)$.} When conditions for \textit{parallel} sampling are not met, we can tune our \textit{parallel} sampling method. For it, denoising at each step $t$ is performed as many times as models are available. For each model $M_i$, frames belonging to a segment generated by another model $M_j,j\neq i$ are unconditionally sampled. This ensures that denoising paths of different conditioning signals do not degenerate.
\end{itemize}

Note that on all sampling schedules, for absolute PE, the attention matrix is nullified outside each individual segment to avoid repeated similarities on the PE outside that particular segment, as shown in Fig. X. For the relative PE, we keep it as is, as we don't care about the sequence length, and restrict the attention to the maximum sequence length seen at training.


==> tables/auto/atthorizon_babel_results.tex <==
\begin{tabular}{lc|cccc|cccc}
\toprule
 & Inf.  & R-prec & FID & Div & MM-Dist  & FID & Div & PJ & AUJ  \\
\midrule
GT & -  & 0.712 & 0.0 & 8.37 & 3.36  & 0.0 & 6.99 & 0.02 & 0.01  \\
50 & RPE  & 0.639 & 1.09 & 7.91 & 3.94  & 1.34 & 7.28 & \textbf{0.04} & 0.26  \\
50 & BPE  & 0.696 & 1.06 & 8.23 & \underline{3.43}  & \underline{1.24} & 7.2 & 0.06 & 0.18  \\
100 & RPE  & 0.639 & \textbf{0.82} & 8.28 & 3.95  & 1.31 & 7.41 & 0.04 & 0.28  \\
100 & BPE  & \underline{0.701} & \underline{1.0} & 8.32 & 3.45  & 1.24 & 7.24 & 0.06 & \underline{0.18}  \\
150 & RPE  & 0.643 & 1.01 & 8.27 & 3.87  & 1.45 & 7.52 & 0.04 & 0.24  \\
150 & BPE  & \textbf{0.704} & 1.25 & 8.42 & \textbf{3.41}  & \textbf{1.24} & 7.23 & 0.07 & \textbf{0.17}  \\
200 & RPE  & 0.6 & 1.52 & 7.87 & 4.16  & 2.67 & 7.3 & \underline{0.04} & 0.35  \\
200 & BPE  & 0.689 & 1.15 & 8.3 & 3.44  & 1.63 & 7.32 & 0.06 & 0.19  \\
\bottomrule
\end{tabular}


==> tables/auto/atthorizon_humanml_results.tex <==
\begin{tabular}{lc|cccc|cccc}
\toprule
 & Inf.  & R-prec & FID & Div & MM-Dist  & FID & Div & PJ & AUJ  \\
\midrule
GT & -  & 0.795 & 0.0 & 9.52 & 2.98  & 0.0 & 9.57 & 0.04 & 0.07  \\
50 & RPE  & 0.575 & 1.02 & 8.99 & 4.27  & 1.77 & 8.78 & \underline{0.04} & 0.69  \\
50 & BPE  & 0.666 & \textbf{0.25} & 9.45 & 3.67  & \underline{1.31} & 8.7 & 0.06 & 0.53  \\
100 & RPE  & 0.594 & 0.98 & 9.03 & 4.27  & 1.51 & 8.86 & 0.04 & 0.56  \\
100 & BPE  & \underline{0.685} & 0.34 & 9.66 & \textbf{3.6}  & 1.98 & 8.53 & 0.06 & 0.54  \\
150 & RPE  & 0.558 & 1.03 & 9.0 & 4.51  & \textbf{1.15} & 8.82 & 0.05 & \underline{0.53}  \\
150 & BPE  & \textbf{0.687} & \underline{0.29} & 9.49 & \underline{3.62}  & 1.47 & 8.77 & 0.06 & \textbf{0.51}  \\
200 & RPE  & 0.527 & 1.34 & 8.91 & 4.67  & 1.9 & 8.77 & \textbf{0.03} & 0.96  \\
200 & BPE  & 0.653 & 0.46 & 9.44 & 3.78  & 2.26 & 8.66 & 0.06 & 0.68  \\
\bottomrule
\end{tabular}


==> tables/auto/babel_scenarios.tex <==
\begin{tabular}{l|cccc|cccc}
\toprule
  & R-prec & FID & Div & MM-Dist  & FID & Div & PJ & AUJ  \\
\midrule
GT  & $0.715^{\pm0.003}$ & $0.00^{\pm0.00}$ & $8.42^{\pm0.15}$ & $3.36^{\pm0.00}$  & $0.00^{\pm0.00}$ & $6.20^{\pm0.06}$ & $0.02^{\pm0.00}$ & $0.00^{\pm0.00}$  \\
\midrule In-distribution \\
\midrule TEACH\_B  & $\underline{0.727}^{\pm0.004}$ & $2.26^{\pm0.03}$ & $8.20^{\pm0.12}$ & $\underline{3.35}^{\pm0.01}$  & $2.77^{\pm0.05}$ & $6.32^{\pm0.07}$ & $1.03^{\pm0.00}$ & $2.20^{\pm0.01}$  \\
TEACH  & $0.665^{\pm0.003}$ & $2.09^{\pm0.03}$ & $8.06^{\pm0.09}$ & $3.73^{\pm0.02}$  & $2.78^{\pm0.06}$ & $6.31^{\pm0.07}$ & $0.07^{\pm0.00}$ & $0.42^{\pm0.01}$  \\
DoubleTake*  & $0.620^{\pm0.006}$ & $3.04^{\pm0.06}$ & $7.49^{\pm0.07}$ & $4.19^{\pm0.02}$  & $3.04^{\pm0.12}$ & $\underline{6.21}^{\pm0.06}$ & $0.28^{\pm0.00}$ & $1.01^{\pm0.01}$  \\
DoubleTake  & $0.682^{\pm0.008}$ & $1.52^{\pm0.03}$ & $7.90^{\pm0.07}$ & $3.67^{\pm0.04}$  & $3.47^{\pm0.08}$ & $6.16^{\pm0.07}$ & $0.17^{\pm0.00}$ & $0.62^{\pm0.01}$  \\
MultiDiffusion  & $0.724^{\pm0.008}$ & $2.00^{\pm0.05}$ & $\underline{8.36}^{\pm0.10}$ & $3.38^{\pm0.02}$  & $6.33^{\pm0.13}$ & $5.91^{\pm0.06}$ & $0.17^{\pm0.00}$ & $0.65^{\pm0.01}$  \\
DiffCollage  & $0.690^{\pm0.006}$ & $1.92^{\pm0.07}$ & $7.92^{\pm0.09}$ & $3.67^{\pm0.02}$  & $4.25^{\pm0.15}$ & $\textbf{6.19}^{\pm0.07}$ & $0.19^{\pm0.01}$ & $0.82^{\pm0.02}$  \\
\midrule SAT  & $0.692^{\pm0.006}$ & $1.85^{\pm0.05}$ & $8.32^{\pm0.12}$ & $3.63^{\pm0.02}$  & $\textbf{1.73}^{\pm0.06}$ & $6.71^{\pm0.07}$ & $\underline{0.05}^{\pm0.00}$ & $\underline{0.11}^{\pm0.01}$  \\
CAT  & $\textbf{0.736}^{\pm0.005}$ & $\underline{1.39}^{\pm0.07}$ & $8.34^{\pm0.09}$ & $\textbf{3.19}^{\pm0.01}$  & $2.42^{\pm0.09}$ & $6.31^{\pm0.05}$ & $\textbf{0.02}^{\pm0.00}$ & $\textbf{0.06}^{\pm0.01}$  \\
PCCAT  & $0.726^{\pm0.006}$ & $\textbf{1.36}^{\pm0.05}$ & $\textbf{8.47}^{\pm0.10}$ & $3.40^{\pm0.03}$  & $\underline{2.26}^{\pm0.08}$ & $6.60^{\pm0.08}$ & $\underline{0.05}^{\pm0.00}$ & $\underline{0.11}^{\pm0.00}$  \\
\midrule Out-of-distribution \\
\midrule TEACH\_B  & $0.680^{\pm0.006}$ & $1.75^{\pm0.04}$ & $8.15^{\pm0.11}$ & $3.51^{\pm0.01}$  & $3.53^{\pm0.06}$ & $6.04^{\pm0.10}$ & $1.14^{\pm0.01}$ & $2.49^{\pm0.01}$  \\
TEACH  & $0.644^{\pm0.004}$ & $2.06^{\pm0.03}$ & $7.94^{\pm0.12}$ & $3.70^{\pm0.01}$  & $4.08^{\pm0.08}$ & $6.00^{\pm0.09}$ & $0.07^{\pm0.00}$ & $0.46^{\pm0.00}$  \\
DoubleTake*  & $0.572^{\pm0.007}$ & $3.78^{\pm0.07}$ & $7.53^{\pm0.12}$ & $4.15^{\pm0.02}$  & $3.83^{\pm0.09}$ & $\textbf{6.12}^{\pm0.07}$ & $0.28^{\pm0.00}$ & $1.07^{\pm0.02}$  \\
DoubleTake  & $0.654^{\pm0.009}$ & $1.65^{\pm0.07}$ & $8.06^{\pm0.08}$ & $3.66^{\pm0.02}$  & $2.98^{\pm0.06}$ & $6.03^{\pm0.07}$ & $0.17^{\pm0.00}$ & $0.66^{\pm0.01}$  \\
MultiDiffusion  & $\underline{0.681}^{\pm0.009}$ & $2.11^{\pm0.06}$ & $\textbf{8.35}^{\pm0.08}$ & $\underline{3.47}^{\pm0.03}$  & $6.97^{\pm0.12}$ & $5.67^{\pm0.05}$ & $0.19^{\pm0.00}$ & $0.71^{\pm0.01}$  \\
DiffCollage  & $0.652^{\pm0.004}$ & $\underline{1.60}^{\pm0.07}$ & $7.91^{\pm0.09}$ & $3.74^{\pm0.01}$  & $4.65^{\pm0.19}$ & $6.00^{\pm0.09}$ & $0.20^{\pm0.00}$ & $0.86^{\pm0.01}$  \\
\midrule SAT  & $0.671^{\pm0.003}$ & $1.81^{\pm0.05}$ & $8.13^{\pm0.11}$ & $3.60^{\pm0.02}$  & $\textbf{2.38}^{\pm0.06}$ & $\underline{6.33}^{\pm0.04}$ & $\underline{0.06}^{\pm0.00}$ & $\underline{0.14}^{\pm0.00}$  \\
CAT  & $\textbf{0.703}^{\pm0.006}$ & $1.78^{\pm0.07}$ & $8.03^{\pm0.10}$ & $\textbf{3.35}^{\pm0.03}$  & $\underline{2.92}^{\pm0.12}$ & $5.92^{\pm0.07}$ & $\textbf{0.02}^{\pm0.00}$ & $\textbf{0.07}^{\pm0.01}$  \\
PCCAT  & $0.679^{\pm0.004}$ & $\textbf{1.26}^{\pm0.06}$ & $\underline{8.16}^{\pm0.08}$ & $3.50^{\pm0.03}$  & $3.17^{\pm0.12}$ & $6.44^{\pm0.09}$ & $0.07^{\pm0.00}$ & $0.17^{\pm0.00}$  \\
\bottomrule
\end{tabular}


==> tables/auto/cfg_babel_results.tex <==
\begin{tabular}{lc|cccc|cccccc}
\toprule
 & CFG  & R-prec & FID & Div & MM-Dist  & FID & Div & Jerk & AUJ & AUJ+ & AUJ-  \\
\midrule
GT & -  & 0.53 & 0.0 & 8.66 & 4.4  & 0.0 & 8.35 & 0.02 & 0.01 & 0.01 & 0.01  \\
\midrule
Ours - AllAbs & 1.00  & 0.39 & 7.02 & 7.14 & 5.84  & 6.55 & 6.82 & 1.95 & 4.46 & 3.85 & 0.62  \\
Ours - AllAbs & 1.25  & 0.42 & 6.22 & 7.21 & 5.65  & 6.08 & 6.88 & 1.99 & 4.47 & 3.92 & 0.54  \\
Ours - AllAbs & 1.50  & 0.43 & 5.71 & 7.28 & 5.51  & 5.73 & 6.95 & 2.02 & 4.47 & 3.99 & 0.48  \\
Ours - AllAbs & 1.75  & 0.45 & 5.31 & 7.37 & 5.39  & 5.57 & 6.95 & 2.05 & 4.44 & 4.06 & 0.38  \\
Ours - AllAbs & 2.0  & 0.45 & 4.97 & 7.4 & 5.31  & 5.31 & 6.96 & 2.07 & 4.37 & 4.1 & 0.27  \\
Ours - AllAbs & 2.50  & 0.47 & 4.29 & 7.51 & 5.15  & 5.06 & 6.92 & 2.08 & 4.31 & 4.26 & 0.05  \\
\midrule
Ours - AllRel & 1.00  & 0.47 & 0.98 & 8.26 & 4.6  & 1.53 & 7.93 & \textbf{0.03} & 0.42 & \textbf{0.01} & 0.41  \\
Ours - AllRel & 1.25  & 0.52 & 0.63 & 8.52 & 4.24  & 1.05 & 7.92 & 0.04 & 0.35 & 0.04 & 0.31  \\
Ours - AllRel & 1.50  & 0.54 & 0.54 & 8.64 & 4.03  & 0.96 & 7.98 & 0.06 & 0.31 & 0.07 & 0.25  \\
Ours - AllRel & 1.75  & 0.56 & 0.54 & 8.69 & 3.89  & 0.93 & 7.99 & 0.07 & 0.26 & 0.1 & 0.17  \\
Ours - AllRel & 2.0  & 0.58 & 0.57 & 8.7 & 3.81  & 0.98 & 7.95 & 0.09 & 0.23 & 0.14 & 0.09  \\
Ours - AllRel & 2.50  & 0.59 & 0.59 & 8.75 & 3.74  & 1.06 & 7.9 & 0.13 & 0.3 & 0.29 & 0.0  \\
\midrule
Ours - Step10 & 1.00  & 0.57 & 0.58 & 8.61 & 3.87  & 1.0 & 7.9 & 0.05 & 0.31 & 0.05 & 0.26  \\
Ours - Step10 & 1.25  & 0.6 & 0.6 & 8.77 & 3.6  & 1.02 & 7.76 & 0.06 & 0.26 & 0.08 & 0.18  \\
Ours - Step10 & 1.50  & 0.62 & 0.68 & 8.84 & 3.48  & 1.1 & 7.71 & 0.08 & \underline{0.23} & 0.13 & 0.1  \\
Ours - Step10 & 1.75  & 0.63 & 0.77 & 8.89 & 3.39  & 1.23 & 7.72 & 0.1 & 0.23 & 0.19 & 0.04  \\
Ours - Step10 & 2.0  & 0.64 & 0.84 & 8.91 & 3.35  & 1.36 & 7.7 & 0.12 & 0.3 & 0.3 & 0.01  \\
Ours - Step10 & 2.50  & 0.64 & 0.99 & 8.94 & \underline{3.33}  & 1.58 & 7.81 & 0.18 & 0.59 & 0.59 & \textbf{0.0}  \\
\bottomrule
\end{tabular}


==> tables/auto/cfg_humanml_results.tex <==
\begin{tabular}{lc|cccc|cccccc}
\toprule
 & CFG  & R-prec & FID & Div & MM-Dist  & FID & Div & Jerk & AUJ & AUJ+ & AUJ-  \\
\midrule
GT & -  & 0.8 & 0.0 & 9.52 & 2.98  & 0.0 & 9.57 & 0.04 & 0.07 & 0.03 & 0.03  \\
DoubleTake & -  & 0.64 & 0.79 & 9.35 & 3.91  & \textbf{1.65} & 8.73 & 0.52 & 2.08 & 1.94 & 0.14  \\
Step10 & 1.0  & 0.55 & 1.3 & 8.7 & 4.39  & 2.6 & 7.79 & \textbf{0.06} & 0.81 & \textbf{0.05} & 0.76  \\
Step10 & 1.25  & 0.59 & 0.88 & 8.88 & 4.11  & 2.14 & 7.99 & \underline{0.08} & 0.74 & \underline{0.09} & 0.65  \\
Step10 & 1.5  & 0.62 & 0.66 & 8.96 & 3.9  & 1.92 & 8.04 & 0.09 & 0.67 & 0.15 & 0.52  \\
Step10 & 1.75  & 0.64 & 0.57 & 9.01 & 3.8  & 1.84 & 8.1 & 0.11 & 0.64 & 0.2 & 0.45  \\
Step10 & 2.0  & 0.66 & 0.55 & 9.25 & 3.73  & \underline{1.77} & 8.2 & 0.12 & 0.59 & 0.24 & 0.35  \\
Step10 & 2.5  & 0.68 & \underline{0.51} & 9.2 & 3.64  & 1.88 & 8.21 & 0.16 & \textbf{0.55} & 0.37 & 0.18  \\
Step10 & 3.0  & \underline{0.69} & \textbf{0.49} & 9.19 & \textbf{3.59}  & 2.01 & 8.16 & 0.19 & \underline{0.58} & 0.51 & 0.07  \\
Step10 & 4.0  & \textbf{0.7} & 0.6 & 9.04 & \underline{3.6}  & 2.47 & 7.97 & 0.27 & 1.01 & 1.01 & \underline{0.0}  \\
Step10 & 5.0  & 0.68 & 0.87 & 8.86 & 3.69  & 3.14 & 7.88 & 0.35 & 1.69 & 1.69 & \textbf{0.0}  \\
\bottomrule
\end{tabular}


==> tables/auto/epochs_babel_results.tex <==
\begin{tabular}{lc|cccc|cccc}
\toprule
 & Epochs  & R-prec & FID & Div & MM-Dist  & FID & Div & PJ & AUJ  \\
\midrule
GT & -  & \textbf{0.712} & \textbf{0.0} & 8.43 & \textbf{3.36}  & \textbf{0.0} & 6.29 & \textbf{0.02} & \textbf{0.0}  \\
qonlymult & 250k  & 0.66 & 2.16 & 8.01 & 3.86  & 3.1 & 6.66 & 0.08 & 0.22  \\
qonlymult & 500k  & \underline{0.699} & 1.18 & 8.26 & \underline{3.4}  & 3.24 & 6.35 & 0.05 & 0.13  \\
qonlymult & 600k  & 0.657 & 1.63 & 8.22 & 3.78  & 4.25 & 6.37 & 0.05 & 0.18  \\
qonlymult & 750k  & 0.689 & 1.53 & 8.09 & 3.59  & 3.27 & 6.64 & 0.06 & \underline{0.12}  \\
qonlymult & 900k  & 0.672 & 1.66 & 8.31 & 3.62  & 3.34 & 6.35 & 0.05 & 0.13  \\
qonlymult & 1M  & 0.698 & 1.39 & 8.4 & 3.43  & 4.38 & 6.35 & \underline{0.05} & 0.14  \\
qonlymult & 1.1M  & 0.679 & 1.26 & 8.37 & 3.58  & 3.93 & 6.52 & 0.06 & 0.15  \\
qonlymult & 1.2M  & 0.693 & 1.35 & 8.31 & 3.47  & 3.42 & 6.34 & 0.05 & 0.15  \\
qonlymult & 1.3M  & 0.693 & 0.97 & 8.29 & 3.5  & 2.58 & 6.44 & 0.06 & 0.13  \\
qonlymult & 1.4M  & 0.674 & \underline{0.88} & 8.22 & 3.65  & \underline{2.28} & 6.44 & 0.06 & 0.13  \\
qonlymult & 1.5M  & 0.675 & 0.91 & 8.36 & 3.6  & 3.02 & 6.44 & 0.05 & 0.13  \\
\bottomrule
\end{tabular}


==> tables/auto/epochs_humanml_results.tex <==
\begin{tabular}{lc|cccc|cccc}
\toprule
 & Epochs  & R-prec & FID & Div & MM-Dist  & FID & Div & Jerk & AUJ  \\
\midrule
qonlymult & 2k  & 0.628 & 0.86 & 9.43 & 4.0  & 3.05 & 8.31 & 0.08 & \underline{0.54}  \\
qonlymult & 3k  & 0.64 & 1.96 & 9.39 & 3.94  & 6.43 & 8.18 & \underline{0.07} & 0.74  \\
qonlymult & 4k  & 0.649 & 0.65 & 9.13 & 3.87  & 2.5 & 8.53 & 0.07 & 0.66  \\
qonlymult & 5k  & \textbf{0.692} & \textbf{0.33} & 9.59 & \textbf{3.58}  & \textbf{1.66} & 8.63 & 0.08 & 0.59  \\
qonlymult & 6k  & \underline{0.681} & \underline{0.64} & 9.25 & \underline{3.61}  & \underline{2.01} & 8.29 & \textbf{0.06} & \textbf{0.52}  \\
\bottomrule
\end{tabular}


==> tables/auto/humanml_scenarios.tex <==
\begin{tabular}{l|cccc|cccc}
\toprule
  & R-prec & FID & Div & MM-Dist  & FID & Div & PJ & AUJ  \\
\midrule
GT  & $0.796^{\pm0.004}$ & $0.00^{\pm0.00}$ & $9.34^{\pm0.08}$ & $2.97^{\pm0.01}$  & $0.00^{\pm0.00}$ & $9.54^{\pm0.15}$ & $0.04^{\pm0.00}$ & $0.07^{\pm0.00}$  \\
\midrule Short sequences \\
\midrule DoubleTake*  & $0.649^{\pm0.012}$ & $\textbf{3.03}^{\pm0.18}$ & $\underline{9.52}^{\pm0.11}$ & $3.72^{\pm0.05}$  & $\underline{3.56}^{\pm0.14}$ & $\underline{8.92}^{\pm0.14}$ & $0.13^{\pm0.01}$ & $0.79^{\pm0.05}$  \\
DoubleTake  & $0.704^{\pm0.022}$ & $4.85^{\pm0.20}$ & $10.01^{\pm0.15}$ & $3.25^{\pm0.09}$  & $4.40^{\pm0.24}$ & $8.88^{\pm0.17}$ & $0.09^{\pm0.00}$ & $0.73^{\pm0.02}$  \\
MultiDiffusion  & $\underline{0.717}^{\pm0.011}$ & $5.49^{\pm0.15}$ & $10.14^{\pm0.17}$ & $\underline{3.23}^{\pm0.07}$  & $4.66^{\pm0.27}$ & $8.68^{\pm0.08}$ & $0.10^{\pm0.00}$ & $0.92^{\pm0.02}$  \\
DiffCollage  & $0.705^{\pm0.012}$ & $4.69^{\pm0.18}$ & $9.73^{\pm0.14}$ & $3.30^{\pm0.04}$  & $4.81^{\pm0.32}$ & $8.49^{\pm0.12}$ & $0.15^{\pm0.01}$ & $1.13^{\pm0.10}$  \\
\midrule SAT  & $\textbf{0.725}^{\pm0.013}$ & $4.79^{\pm0.16}$ & $9.63^{\pm0.21}$ & $\textbf{3.09}^{\pm0.05}$  & $4.75^{\pm0.30}$ & $8.38^{\pm0.15}$ & $\textbf{0.04}^{\pm0.00}$ & $\underline{0.40}^{\pm0.03}$  \\
CAT  & $0.624^{\pm0.010}$ & $\underline{4.17}^{\pm0.18}$ & $\textbf{9.21}^{\pm0.14}$ & $4.00^{\pm0.09}$  & $3.86^{\pm0.24}$ & $8.47^{\pm0.18}$ & $0.05^{\pm0.00}$ & $\textbf{0.36}^{\pm0.04}$  \\
FlowMDM  & $0.714^{\pm0.015}$ & $4.75^{\pm0.26}$ & $9.90^{\pm0.20}$ & $3.31^{\pm0.06}$  & $\textbf{3.17}^{\pm0.17}$ & $\textbf{9.03}^{\pm0.14}$ & $\textbf{0.04}^{\pm0.00}$ & $0.59^{\pm0.04}$  \\
\midrule Medium sequences \\
\midrule DoubleTake*  & $0.644^{\pm0.009}$ & $2.18^{\pm0.08}$ & $9.18^{\pm0.12}$ & $3.72^{\pm0.04}$  & $\underline{3.34}^{\pm0.30}$ & $\textbf{8.73}^{\pm0.12}$ & $0.14^{\pm0.00}$ & $0.70^{\pm0.03}$  \\
DoubleTake  & $0.642^{\pm0.014}$ & $2.34^{\pm0.05}$ & $9.59^{\pm0.09}$ & $3.79^{\pm0.05}$  & $5.42^{\pm0.30}$ & $\underline{8.61}^{\pm0.11}$ & $0.12^{\pm0.00}$ & $0.83^{\pm0.02}$  \\
MultiDiffusion  & $\underline{0.673}^{\pm0.007}$ & $3.22^{\pm0.10}$ & $9.91^{\pm0.07}$ & $\underline{3.54}^{\pm0.04}$  & $6.24^{\pm0.34}$ & $8.11^{\pm0.12}$ & $0.10^{\pm0.00}$ & $1.14^{\pm0.01}$  \\
DiffCollage  & $0.661^{\pm0.010}$ & $2.03^{\pm0.07}$ & $\textbf{9.38}^{\pm0.10}$ & $3.60^{\pm0.04}$  & $4.95^{\pm0.27}$ & $8.13^{\pm0.09}$ & $0.14^{\pm0.00}$ & $\textbf{0.66}^{\pm0.05}$  \\
\midrule SAT  & $\textbf{0.702}^{\pm0.013}$ & $\textbf{1.73}^{\pm0.06}$ & $\underline{9.27}^{\pm0.10}$ & $\textbf{3.35}^{\pm0.04}$  & $\textbf{2.70}^{\pm0.17}$ & $8.12^{\pm0.12}$ & $\textbf{0.03}^{\pm0.00}$ & $\underline{0.67}^{\pm0.03}$  \\
CAT  & $0.626^{\pm0.013}$ & $\underline{1.88}^{\pm0.08}$ & $9.19^{\pm0.10}$ & $4.00^{\pm0.04}$  & $3.46^{\pm0.15}$ & $8.38^{\pm0.08}$ & $\textbf{0.03}^{\pm0.00}$ & $0.81^{\pm0.04}$  \\
FlowMDM  & $0.669^{\pm0.012}$ & $3.18^{\pm0.15}$ & $9.68^{\pm0.08}$ & $3.55^{\pm0.04}$  & $4.18^{\pm0.43}$ & $8.52^{\pm0.07}$ & $0.04^{\pm0.00}$ & $0.86^{\pm0.03}$  \\
\midrule Long sequences \\
\midrule DoubleTake*  & $0.616^{\pm0.006}$ & $2.51^{\pm0.09}$ & $\underline{8.77}^{\pm0.08}$ & $4.09^{\pm0.03}$  & $\underline{3.38}^{\pm0.18}$ & $\underline{8.50}^{\pm0.11}$ & $0.89^{\pm0.02}$ & $3.52^{\pm0.07}$  \\
DoubleTake  & $0.605^{\pm0.006}$ & $4.07^{\pm0.13}$ & $8.19^{\pm0.11}$ & $4.18^{\pm0.01}$  & $8.45^{\pm0.33}$ & $7.79^{\pm0.12}$ & $0.81^{\pm0.02}$ & $3.04^{\pm0.07}$  \\
MultiDiffusion  & $0.569^{\pm0.012}$ & $5.02^{\pm0.15}$ & $8.07^{\pm0.07}$ & $4.49^{\pm0.05}$  & $8.56^{\pm0.32}$ & $7.91^{\pm0.10}$ & $0.23^{\pm0.01}$ & $1.16^{\pm0.01}$  \\
DiffCollage  & $0.557^{\pm0.008}$ & $5.79^{\pm0.13}$ & $7.75^{\pm0.09}$ & $4.61^{\pm0.02}$  & $9.00^{\pm0.36}$ & $7.75^{\pm0.09}$ & $0.38^{\pm0.01}$ & $5.04^{\pm0.14}$  \\
\midrule SAT  & $\underline{0.661}^{\pm0.005}$ & $\underline{2.21}^{\pm0.06}$ & $8.23^{\pm0.09}$ & $\textbf{3.72}^{\pm0.02}$  & $5.23^{\pm0.26}$ & $7.67^{\pm0.14}$ & $\underline{0.05}^{\pm0.00}$ & $\textbf{0.30}^{\pm0.03}$  \\
CAT  & $0.617^{\pm0.008}$ & $4.54^{\pm0.09}$ & $8.08^{\pm0.08}$ & $4.10^{\pm0.02}$  & $7.18^{\pm0.23}$ & $7.98^{\pm0.09}$ & $\textbf{0.04}^{\pm0.00}$ & $0.53^{\pm0.02}$  \\
FlowMDM  & $\textbf{0.666}^{\pm0.012}$ & $\textbf{1.93}^{\pm0.08}$ & $\textbf{8.81}^{\pm0.09}$ & $\underline{3.81}^{\pm0.04}$  & $\textbf{2.85}^{\pm0.22}$ & $\textbf{8.54}^{\pm0.11}$ & $0.08^{\pm0.00}$ & $\underline{0.45}^{\pm0.03}$  \\
\bottomrule
\end{tabular}


==> tables/auto/steps_babel_results.tex <==
\begin{tabular}{lc|cccc|cccc}
\toprule
 & Steps  & R-prec $\uparrow{}$ & FID $\downarrow{}$ & Div $\rightarrow$ & MM-Dist $\downarrow{}$  & FID $\downarrow{}$ & Div $\rightarrow{}$ & PJ $\rightarrow{}$ & AUJ $\downarrow{}$  \\
\midrule
GT & -  & $0.712^{\pm0.004}$ & $0.00^{\pm0.00}$ & $8.43^{\pm0.19}$ & $3.36^{\pm0.00}$  & $0.00^{\pm0.00}$ & $6.29^{\pm0.15}$ & $0.02^{\pm0.00}$ & $0.00^{\pm0.00}$  \\
Ours & 0  & $0.639^{\pm0.012}$ & $\textbf{0.82}^{\pm0.04}$ & $8.28^{\pm0.34}$ & $3.95^{\pm0.05}$  & $\textbf{2.14}^{\pm0.02}$ & $6.44^{\pm0.05}$ & $\textbf{0.04}^{\pm0.00}$ & $0.16^{\pm0.01}$  \\
Ours & 5  & $0.681^{\pm0.006}$ & $\underline{0.91}^{\pm0.05}$ & $8.26^{\pm0.11}$ & $3.70^{\pm0.01}$  & $\underline{2.41}^{\pm0.17}$ & $6.41^{\pm0.05}$ & $\underline{0.05}^{\pm0.00}$ & $0.14^{\pm0.01}$  \\
Ours & 6  & $0.680^{\pm0.005}$ & $\underline{0.91}^{\pm0.06}$ & $8.28^{\pm0.24}$ & $3.65^{\pm0.02}$  & $2.44^{\pm0.14}$ & $6.44^{\pm0.16}$ & $\underline{0.05}^{\pm0.00}$ & $0.14^{\pm0.00}$  \\
Ours & 7  & $0.685^{\pm0.002}$ & $0.93^{\pm0.06}$ & $8.27^{\pm0.23}$ & $3.60^{\pm0.02}$  & $2.44^{\pm0.10}$ & $\underline{6.40}^{\pm0.22}$ & $\underline{0.05}^{\pm0.00}$ & $\underline{0.13}^{\pm0.00}$  \\
Ours & 8  & $0.693^{\pm0.006}$ & $0.95^{\pm0.08}$ & $8.27^{\pm0.23}$ & $3.56^{\pm0.02}$  & $2.51^{\pm0.13}$ & $6.45^{\pm0.19}$ & $\underline{0.05}^{\pm0.00}$ & $\underline{0.13}^{\pm0.00}$  \\
Ours & 9  & $0.692^{\pm0.004}$ & $0.96^{\pm0.08}$ & $8.27^{\pm0.24}$ & $3.53^{\pm0.02}$  & $2.55^{\pm0.15}$ & $6.43^{\pm0.17}$ & $\underline{0.05}^{\pm0.00}$ & $\underline{0.13}^{\pm0.00}$  \\
Ours & 10  & $0.693^{\pm0.008}$ & $0.97^{\pm0.09}$ & $8.29^{\pm0.24}$ & $3.50^{\pm0.02}$  & $2.58^{\pm0.16}$ & $6.44^{\pm0.16}$ & $0.06^{\pm0.00}$ & $\underline{0.13}^{\pm0.00}$  \\
Ours & 12.5  & $0.701^{\pm0.008}$ & $1.00^{\pm0.09}$ & $8.32^{\pm0.25}$ & $3.45^{\pm0.02}$  & $2.64^{\pm0.16}$ & $6.44^{\pm0.08}$ & $0.06^{\pm0.00}$ & $\textbf{0.12}^{\pm0.01}$  \\
Ours & 15  & $0.704^{\pm0.008}$ & $1.02^{\pm0.08}$ & $8.37^{\pm0.24}$ & $3.44^{\pm0.04}$  & $2.69^{\pm0.18}$ & $6.44^{\pm0.04}$ & $0.07^{\pm0.00}$ & $0.14^{\pm0.01}$  \\
Ours & 17.5  & $0.705^{\pm0.007}$ & $1.03^{\pm0.08}$ & $\textbf{8.38}^{\pm0.21}$ & $3.42^{\pm0.03}$  & $2.73^{\pm0.18}$ & $6.43^{\pm0.04}$ & $0.07^{\pm0.00}$ & $0.15^{\pm0.02}$  \\
Ours & 20  & $0.705^{\pm0.005}$ & $1.04^{\pm0.08}$ & $\textbf{8.38}^{\pm0.21}$ & $3.41^{\pm0.03}$  & $2.76^{\pm0.18}$ & $6.44^{\pm0.05}$ & $0.07^{\pm0.00}$ & $0.16^{\pm0.02}$  \\
Ours & 25  & $0.706^{\pm0.005}$ & $1.05^{\pm0.04}$ & $8.33^{\pm0.22}$ & $3.41^{\pm0.03}$  & $2.79^{\pm0.11}$ & $6.51^{\pm0.15}$ & $0.08^{\pm0.00}$ & $0.19^{\pm0.01}$  \\
Ours & 30  & $0.709^{\pm0.002}$ & $1.06^{\pm0.05}$ & $8.34^{\pm0.21}$ & $3.40^{\pm0.03}$  & $2.81^{\pm0.12}$ & $6.51^{\pm0.17}$ & $0.09^{\pm0.00}$ & $0.22^{\pm0.00}$  \\
Ours & 50  & $0.710^{\pm0.002}$ & $1.09^{\pm0.05}$ & $8.34^{\pm0.19}$ & $3.38^{\pm0.02}$  & $2.89^{\pm0.14}$ & $6.53^{\pm0.22}$ & $0.13^{\pm0.01}$ & $0.33^{\pm0.02}$  \\
Ours & 60  & $0.712^{\pm0.004}$ & $1.10^{\pm0.04}$ & $8.34^{\pm0.18}$ & $3.38^{\pm0.02}$  & $2.93^{\pm0.13}$ & $6.53^{\pm0.22}$ & $0.16^{\pm0.00}$ & $0.40^{\pm0.01}$  \\
Ours & 70  & $0.713^{\pm0.002}$ & $1.10^{\pm0.04}$ & $8.34^{\pm0.17}$ & $3.37^{\pm0.02}$  & $2.98^{\pm0.13}$ & $6.52^{\pm0.22}$ & $0.20^{\pm0.01}$ & $0.48^{\pm0.01}$  \\
Ours & 80  & $0.712^{\pm0.004}$ & $1.11^{\pm0.04}$ & $8.35^{\pm0.17}$ & $3.37^{\pm0.02}$  & $3.03^{\pm0.12}$ & $6.52^{\pm0.21}$ & $0.24^{\pm0.00}$ & $0.58^{\pm0.01}$  \\
Ours & 90  & $\underline{0.716}^{\pm0.003}$ & $1.11^{\pm0.04}$ & $8.35^{\pm0.17}$ & $\underline{3.35}^{\pm0.02}$  & $3.11^{\pm0.12}$ & $6.52^{\pm0.20}$ & $0.30^{\pm0.00}$ & $0.72^{\pm0.01}$  \\
Ours & 100  & $\textbf{0.718}^{\pm0.006}$ & $1.17^{\pm0.05}$ & $8.27^{\pm0.27}$ & $\textbf{3.31}^{\pm0.00}$  & $3.06^{\pm0.03}$ & $\textbf{6.31}^{\pm0.09}$ & $1.78^{\pm0.02}$ & $3.66^{\pm0.04}$  \\
\bottomrule
\end{tabular}


==> tables/auto/steps_humanml_results.tex <==
\begin{tabular}{lc|cccc|cccc}
\toprule
 & Steps  & R-prec $\uparrow{}$ & FID $\downarrow{}$ & Div $\rightarrow$ & MM-Dist $\downarrow{}$  & FID $\downarrow{}$ & Div $\rightarrow{}$ & PJ $\rightarrow{}$ & AUJ $\downarrow{}$  \\
\midrule
GT & -  & $0.795^{\pm0.007}$ & $0.00^{\pm0.00}$ & $9.52^{\pm0.31}$ & $2.98^{\pm0.02}$  & $0.00^{\pm0.00}$ & $9.57^{\pm0.15}$ & $0.04^{\pm0.00}$ & $0.07^{\pm0.00}$  \\
Ours & 0  & $0.558^{\pm0.002}$ & $1.03^{\pm0.04}$ & $9.00^{\pm0.18}$ & $4.51^{\pm0.04}$  & $\textbf{1.15}^{\pm0.06}$ & $\textbf{8.82}^{\pm0.11}$ & $\textbf{0.05}^{\pm0.00}$ & $0.53^{\pm0.01}$  \\
Ours & 5  & $0.685^{\pm0.004}$ & $\textbf{0.27}^{\pm0.03}$ & $9.47^{\pm0.23}$ & $3.63^{\pm0.02}$  & $\underline{1.40}^{\pm0.11}$ & $8.76^{\pm0.07}$ & $\underline{0.06}^{\pm0.00}$ & $\textbf{0.50}^{\pm0.01}$  \\
Ours & 6  & $0.687^{\pm0.007}$ & $\underline{0.29}^{\pm0.03}$ & $9.49^{\pm0.22}$ & $3.62^{\pm0.02}$  & $1.47^{\pm0.12}$ & $8.77^{\pm0.10}$ & $\underline{0.06}^{\pm0.00}$ & $\underline{0.51}^{\pm0.01}$  \\
Ours & 7  & $0.688^{\pm0.006}$ & $0.30^{\pm0.02}$ & $\textbf{9.52}^{\pm0.20}$ & $3.62^{\pm0.02}$  & $1.51^{\pm0.11}$ & $\underline{8.78}^{\pm0.07}$ & $0.07^{\pm0.00}$ & $0.53^{\pm0.01}$  \\
Ours & 8  & $0.690^{\pm0.005}$ & $0.31^{\pm0.02}$ & $\underline{9.54}^{\pm0.19}$ & $3.62^{\pm0.02}$  & $1.56^{\pm0.09}$ & $8.75^{\pm0.09}$ & $0.07^{\pm0.00}$ & $0.55^{\pm0.01}$  \\
Ours & 9  & $0.685^{\pm0.004}$ & $0.32^{\pm0.02}$ & $9.57^{\pm0.23}$ & $3.60^{\pm0.03}$  & $1.58^{\pm0.06}$ & $8.59^{\pm0.14}$ & $0.07^{\pm0.00}$ & $0.57^{\pm0.02}$  \\
Ours & 10  & $0.692^{\pm0.003}$ & $0.33^{\pm0.02}$ & $9.59^{\pm0.23}$ & $3.58^{\pm0.01}$  & $1.66^{\pm0.12}$ & $8.63^{\pm0.21}$ & $0.08^{\pm0.00}$ & $0.59^{\pm0.01}$  \\
Ours & 12.5  & $0.691^{\pm0.005}$ & $0.34^{\pm0.01}$ & $9.55^{\pm0.04}$ & $3.59^{\pm0.01}$  & $1.60^{\pm0.10}$ & $8.66^{\pm0.09}$ & $0.08^{\pm0.00}$ & $0.65^{\pm0.02}$  \\
Ours & 15  & $0.693^{\pm0.003}$ & $0.36^{\pm0.01}$ & $9.55^{\pm0.24}$ & $3.58^{\pm0.01}$  & $1.75^{\pm0.05}$ & $8.61^{\pm0.07}$ & $0.09^{\pm0.00}$ & $0.70^{\pm0.02}$  \\
Ours & 17.5  & $0.692^{\pm0.002}$ & $0.37^{\pm0.02}$ & $9.61^{\pm0.20}$ & $3.56^{\pm0.01}$  & $1.81^{\pm0.10}$ & $8.56^{\pm0.19}$ & $0.10^{\pm0.00}$ & $0.70^{\pm0.01}$  \\
Ours & 20  & $0.696^{\pm0.001}$ & $0.38^{\pm0.02}$ & $9.63^{\pm0.20}$ & $3.55^{\pm0.01}$  & $1.85^{\pm0.10}$ & $8.55^{\pm0.18}$ & $0.11^{\pm0.00}$ & $0.72^{\pm0.01}$  \\
Ours & 25  & $0.693^{\pm0.004}$ & $0.38^{\pm0.02}$ & $9.71^{\pm0.24}$ & $3.55^{\pm0.02}$  & $1.80^{\pm0.04}$ & $8.67^{\pm0.07}$ & $0.13^{\pm0.01}$ & $0.77^{\pm0.02}$  \\
Ours & 30  & $0.695^{\pm0.006}$ & $0.40^{\pm0.02}$ & $9.72^{\pm0.25}$ & $3.55^{\pm0.02}$  & $1.84^{\pm0.04}$ & $8.66^{\pm0.06}$ & $0.14^{\pm0.00}$ & $0.80^{\pm0.02}$  \\
Ours & 40  & $0.694^{\pm0.001}$ & $0.43^{\pm0.02}$ & $9.63^{\pm0.15}$ & $\underline{3.54}^{\pm0.02}$  & $1.90^{\pm0.11}$ & $8.61^{\pm0.05}$ & $0.16^{\pm0.01}$ & $0.87^{\pm0.03}$  \\
Ours & 50  & $0.692^{\pm0.008}$ & $0.43^{\pm0.02}$ & $9.65^{\pm0.18}$ & $3.56^{\pm0.01}$  & $2.06^{\pm0.11}$ & $8.57^{\pm0.13}$ & $0.18^{\pm0.00}$ & $0.92^{\pm0.00}$  \\
Ours & 60  & $0.692^{\pm0.008}$ & $0.44^{\pm0.02}$ & $9.66^{\pm0.18}$ & $3.56^{\pm0.01}$  & $2.11^{\pm0.12}$ & $8.56^{\pm0.12}$ & $0.20^{\pm0.01}$ & $0.96^{\pm0.01}$  \\
Ours & 70  & $0.695^{\pm0.007}$ & $0.44^{\pm0.02}$ & $9.65^{\pm0.13}$ & $3.56^{\pm0.02}$  & $1.98^{\pm0.09}$ & $8.50^{\pm0.09}$ & $0.23^{\pm0.01}$ & $1.01^{\pm0.01}$  \\
Ours & 80  & $0.694^{\pm0.008}$ & $0.47^{\pm0.03}$ & $9.68^{\pm0.19}$ & $3.56^{\pm0.01}$  & $2.17^{\pm0.12}$ & $8.56^{\pm0.12}$ & $0.24^{\pm0.00}$ & $1.05^{\pm0.01}$  \\
Ours & 90  & $\underline{0.697}^{\pm0.010}$ & $0.49^{\pm0.03}$ & $9.70^{\pm0.19}$ & $3.55^{\pm0.01}$  & $2.21^{\pm0.12}$ & $8.57^{\pm0.12}$ & $0.26^{\pm0.00}$ & $1.10^{\pm0.01}$  \\
Ours & 100  & $\textbf{0.701}^{\pm0.011}$ & $0.64^{\pm0.07}$ & $9.88^{\pm0.28}$ & $\textbf{3.53}^{\pm0.05}$  & $2.52^{\pm0.07}$ & $8.40^{\pm0.13}$ & $1.39^{\pm0.02}$ & $3.31^{\pm0.03}$  \\
\bottomrule
\end{tabular}

